Anatomy of a Digital Bubble: Lessons Learned from the NFT and Metaverse Frenzy

In the past few years, "metaverse" and "non-fungible tokens (NFT)" have become buzzwords, and the prices of related assets have exhibited large fluctuations. Are those characteristic of a speculative bubble? In this paper, we attempt to answer this question, and better understand the underlying economic dynamics. We look at Decentraland, a virtual world platform where land parcels are sold as NFT collections. We find that initially, land prices followed traditional real estate pricing models - in particular, value decreased with distance from the most desirable areas - suggesting Decentraland behaved much like a virtual city. However, these real estate pricing models stopped applying when both the metaverse and NFTs gained increased popular attention and enthusiasm in 2021, suggesting a new driving force for the underlying asset prices. At that time, following a substantial rise in NFT market values, short-term holders of multiple parcels began to take major selling positions in the Decentraland market, which hints that, rather than building a metaverse community, early Decentraland investors preferred to cash out when land valuations became inflated. Our analysis also shows that while the majority of buyers are new entrants to the market (many of whom joined during the bubble), liquidity (i.e., parcels) was mostly provided by early adopters selling, which caused stark differences in monetary gains. Early adopters made money - more than 10,000 USD on average per parcel sold - but users who joined later typically made no profit or even incurred losses in the order of 1,000 USD per parcel. Unlike established markets such as financial and real estate markets, newly emergent digital marketplaces are mostly self-regulated. As a result, the significant financial risks we identify indicate a strong need for establishing appropriate standards of business conduct and improving user awareness.

==> copyright.tex <==

\begin{minipage}[t]{\textwidth}
\end{minipage}
\vfill
\begin{minipage}[b]{\textwidth}
\textcopyright Daisuke Kawai, 2024. All Rights Reserved.\\
%\textit{The views and conclusions in this document are those of the author and should not be interpreted as representing any view or conclusion, either expressed or implied, of any sponsoring institution or any other entity.}
\end{minipage}

==> decentraland/alt-text.tex <==
Figure 1: \Description[Investor coverage analysis]{Number of collected investors and the lowest rank in our dataset in April 2021}
Figure 2: \Description[Daily Bitcoin price]{Daily BTC price in USDT in April 2021}
Figure 3: \Description[Per-investor number of followers and followees]{Complementary cumulative density function (cCDF) for the per-investor number of follower-investors and followee-investors}
Figure 4: \Description[Number of \#HODL tweets]{Number of \#HODL tweets in April and May 2021}
Figure 5: \Description[Number of dip tweets]{Number of dip tweets in April and May 2021}
Figure 6: \Description[Number of moon tweets]{Number of moon tweets in April and May 2021}
Figure 7: \Description[Number of \#blockchain tweets]{Number of \#blockchain tweets in April and May 2021}
Figure 8: \Description[Number of storm tweets]{Number of storm tweets in April and May 2021}
Figure 9: \Description[CDF plot of advocates' Spearman's rank correlation coefficients]{CDF plot of advocates' Spearman's rank correlation coefficients in 4/3-4/9, 4/10-4/16, 4/17-4/23, and 4/24-4/30}
Figure 10: \Description[Language-use distribution]{Language distribution of investors with Twitter accounts}
Figure 11: \Description[Top 10 cryptocurrencies in open interest]{Ratio of open interest for the top 10 cryptocurrencies in April 2021}
Figure 12: \Description[CDF plot of followers' Spearman's rank correlation coefficients]{CDF plot of followers' Spearman's rank correlation coefficients in 4/3-4/9, 4/10-4/16, 4/17-4/23, and 4/24-4/30}

==> decentraland/third_party_markets.tex <==
\section{Third-party marketplaces}
\label{appx:third_parth}

This section summarizes the third-party marketplaces we consider in this work.
We collect transactions that interact with contract addresses on the Ethereum blockchain listed in Table~\ref{tab:third_party_address}.

\begin{threeparttable}[htbp]
    \centering
    \caption{Third-party marketplaces}
    \begin{tabular}{cl} \toprule
    Marketplace & \multicolumn{1}{c}{Contract address} \\ \midrule
        OpenSea\tnote{1}
        & 0x7Be8076f4EA4A4AD08075C2508e481d6C946D12b \\
        & 0x00000000006c3852cbEf3e08E8dF289169EdE581 \\
        & 0x00000000000006c7676171937C444f6BDe3D6282 \\
        & 0x0000000000000aD24e80fd803C6ac37206a45f15 \\
        & 0x00000000000001ad428e4906aE43D8F9852d0dD6 \\
        & 0x00000000000000ADc04C56Bf30aC9d3c0aAF14dC \vspace{3pt} \\
        LooksRare\tnote{2}
        & 0x59728544B08AB483533076417FbBB2fD0B17CE3a \\
        & 0x0000000000E655fAe4d56241588680F86E3b2377 \vspace{3pt} \\
        Rarible\tnote{3}
        & 0xcd4EC7b66fbc029C116BA9Ffb3e59351c20B5B06 \\
        & 	0x9757F2d2b135150BBeb65308D4a91804107cd8D6 \vspace{3pt} \\
        X2Y2\tnote{4}
        & 0x74312363e45DCaBA76c59ec49a7Aa8A65a67EeD3
        \\ \bottomrule
    \end{tabular}
    \begin{tablenotes}
      \footnotesize 
      \item[1] \url{https://opensea.io/}
      \item[2] \url{https://looksrare.org/} 
      \item[3] \url{https://rarible.com/}
      \item[4] \url{https://x2y2.io/}
    \end{tablenotes}
    \label{tab:third_party_address}
\end{threeparttable}

